Cinema Darkroom: A Deferred Rendering Framework for Large-Scale Datasets

This paper presents a framework that fully leverages the advantages of a deferred rendering approach for the interactive visualization of large-scale datasets. Geometry buffers (G-Buffers) are generated and stored in situ, and shading is performed post hoc in an interactive image-based rendering front end. This decoupled framework has two major advantages. First, the G-Buffers only need to be computed and stored once---which corresponds to the most expensive part of the rendering pipeline. Second, the stored G-Buffers can later be consumed in an image-based rendering front end that enables users to interactively adjust various visualization parameters---such as the applied color map or the strength of ambient occlusion---where suitable choices are often not known a priori. This paper demonstrates the use of Cinema Darkroom on several real-world datasets, highlighting CD's ability to effectively decouple the complexity and size of the dataset from its visualization.

==> figures/turb/turb.tex <==
\renewcommand{\scaleX}{2.2}
\renewcommand{\scaleY}{1}

\renewcommand{\subfigure}[4]{
    \setlength{\fboxsep}{0pt}
    \node at (#1,#2) {
        \includegraphics[width=0.33\textwidth]{#3}
    };
    \node at (#1,#2-2.7) {#4};
}

\begin{figure}
    \begin{center}
        \hspace*{-30em}%
        \begin{tikzpicture}[xscale=\scaleX,yscale=\scaleY]
            \subfigure{0}{0}{./figures/turb/turb.jpg}{};
        \end{tikzpicture}%
        \hspace*{-30em}\vspace*{-2em}
    \end{center}

    \caption{
        This figure shows individual contours (encoded by color) for enstrophy value $2$ of an isotropic turbulence simulation~\cite{openSciVisDataSets}.
        To distinguish between individual features in such a cluttered view, the visualization needs to incorporate depth cues in the form of shadows.
        To provide such depth cues, one can render in situ the entire depicted scene via path tracing to compute global illumination based on a physical-lightning model.
        However, CD can approximate global illumination post hoc via SSAO and a single depth buffer, which requires far less computational effort.
        \edit{Moreover, physical based rendering is restricted to the actual model of light transport, whereas SSAO can also achieve illustrative effects; e.g., by darkening regions around depth discontinuities to enhance spatial perception.}\vspace*{2em}\\
        {\fontfamily{ptm}\selectfont
        \fontsize{9}{9}\selectfont
        However, CD is currently limited to G-Buffers that depict fully opaque geometry.
        This notably excludes post hoc volume rendering (except in its most basic form of directly storing color images in situ).
        To address this issue, other techniques such as the \emph{Explorable Images} approach~\cite{tikhonova2010explorable} or generative models~\cite{berger2018generative} need to be investigated if they
        can be integrated in a deferred rendering pipeline.
        Finally, CD is designed to be easily extendable and we plan to include in future work more image-based shading techniques such as image-space line integral convolution~\cite{Huang2012}, Scalable Ambient Obscurance~\cite{mcguire2012scalable}, and SSAO optimized for particle visualization~\cite{engelke2019autonomous,grottel2014megamol,eichelbaum2013pointao}.\vspace*{-0.8em}}
    }

    \label{fig_turb}
\end{figure}

